Avoiding Inference Heuristics in Few-shot Prompt-based Finetuning

Recent prompt-based approaches allow pretrained language models to achieve strong performances on few-shot finetuning by reformulating downstream tasks as a language modeling problem. In this work, we demonstrate that, despite its advantages on low data regimes, finetuned prompt-based models for sentence pair classification tasks still suffer from a common pitfall of adopting inference heuristics based on lexical overlap, e.g., models incorrectly assuming a sentence pair is of the same meaning because they consist of the same set of words. Interestingly, we find that this particular inference heuristic is significantly less present in the zero-shot evaluation of the prompt-based model, indicating how finetuning can be destructive to useful knowledge learned during the pretraining. We then show that adding a regularization that preserves pretraining weights is effective in mitigating this destructive tendency of few-shot finetuning. Our evaluation on three datasets demonstrates promising improvements on the three corresponding challenge datasets used to diagnose the inference heuristics.

==> comments.tex <==
% Pre-trained Language Models (PLM), e.g., BERT/RoBERTa, are shown to achieve remarkable few-shot learning performance when finetuned on only a handful input text reformulated as cloze questions, known as prompt. In this work, we demonstrate that for sentence pair classification tasks, these models are still especially prone to adopt syntactic heuristics. That is, ... . However, this tendency only appears as more data is seen. To mitigate this, we propose ... We evaluate on and show its effectiveness on three challenge datasets.  

% However, it remains unclear whether the reported results are achieved from robust generalization or model simply adopting inference heuristics, i.e., shortcuts which work well on the majority of the test cases \comment{but fail on OOD}. In this work, we systematically measure the few-shot learners across different data regimes and augmented with varying amount of examples that are counterfactual to the heuristics. We find that \textbf{(1)} zero-shot PLMs, as shown by the non-trivial performance on the diagnostic datasets (e.g., HANS, PAWS), do not blindly employ heuristics (in certain sub-cases they even perform better than fully fine-tuned counterparts). \textbf{(2)} However, once prompt-based PLMs are fine-tuned using more labeled examples (under low data regime), they started to adopt heuristics and severely degrade the diagnostics performance. \textbf{(3)} We conclude that prompt-based finetuning models are especially prone to catastrophic forgetting of the knowledge learned during pre-training and show that continual learning method, i.e., Elastic Weight Consolidation, is effective in improving the target dataset performance while mitigating the adoption of heuristics. \comment{Abstract still to long. Might as well include: our findings call for improved few-shot data curation and training procedure that takes into models robustness related to inference heuristics; fine-grained evaluation of few-shot models}

% \paragraph{Motivation}\comment{:} A common approach for adapting Pre-trained Language Models (PLM) \cite{devlin-etal-2019-bert} for downstream tasks is to add a task-specific head on the last layer and fine-tune the entire model on the labeled training data. Recently, researchers demonstrated that powerful language modeling ability of PLMs can be directly harnessed for other tasks by reformulating task' instances into cloze questions. The natural language prompt allows PLMs to predict the targeted labels with limited or even no labeled examples \cite{schick2020exploiting} \comment{Add citations to GPT-2/3, and T5 model Raffel et al}.

% \paragraph{Problem statement}\comment{:} While promising, earlier work suggest that models learn on small fraction of the training data are more likely to learn simple patterns (\comment{maybe also discuss about inference heuristics here}) that work well on the majority of easier test cases \cite{krymolowski-2002-distinguishing, utama-etal-2020-towards}. \comment{Discuss how the prompt formulation provides the model with non-trivial initialization in learning the task. We are interested to study whether this good initial point may impact models' tendency for learning simple inference heuristics.}
% % it is interesting to see if prompt-based PLMs leaner fall into the same issue

% Specifically, we question whether data efficiency shown by the prompt-based few-shot learners leads to model generalizing better from the limited number of examples that counteract some known heuristics, e.g., lexical overlap heuristic in NLI \cite{mccoy-etal-2019-right}. However, we should expect that in the few-shot learning setting, the small training data is unlikely to include these counterfactual examples to the heuristics. Studying prompt-based model finetuning robustness against heuristics should then be performed under controlled number counterfactual examples in the training data. \comment{Argue using the recent finding that counterfactual examples are needed to tap into the corresponding lingustic information extracted during the pre-training.}


% \paragraph{What do we do} Hypotheses and experimental plans in this work are listed in the folowing:
% \begin{itemize}
%     \item The \textit{missed connection hypothesis} introduced by \citet{min-etal-2020-syntactic} suggests that PLMs extract relevant information during pre-training, but fails to use it because the number of evidence that supports inference heuristics overwhelmingly outweighs the examples that counteract them (counterfactuals). Prompt-based approach which allows PLMs to perform task directly without learning from the \comment{task-specific} heuristics-supporting evidence might avoid adopting heuristics, and perform well in the diagnostic datasets.
%     \item Prompt-based finetuning offer better data efficiency, achieving higher performance on standard benchmark evaluations with much less training data. As we fine-tune prompt-based PLMs on more data, it is more likely that the model would be exposed to examples that either \textit{support} or \textit{counteract} the heuristics. The counterfactuals are most likely to be the minority. The natural question to ask is how the data efficiency of prompt-based PLM play a role in learning from this small number of counterfactuals, in the face of the majority heuristics-supporting counterparts. There are now two possibilities: (1) Prompt-based models learn efficiently from the available counterfactuals and avoid adopting heuristics; (2) models still incline to adopt the heuristics from the \textit{supports}\footnote{For now we refer heuristics-supporting examples as supports} examples. Based on the validation of the previous hypothesis, (2) would mean that if the zero-shot models performs well originally in the diagnostic evaluation, they then suffer from 'catastrophic forgetting' and degrades the performance during diagnostic evaluation. (1) means that models obtain improvement in the diagnostic data regardless of the starting point. 
%     \item Assuming that the small examples for finetuning contain supports and especially counterfactuals might not be realistic. In order to measure prompt-based models ability to learn from the minority examples, we need to control the presence of the corresponding examples. We could therefore augment the small training examples with some examples that are guaranteed to either support or counteract the considered heuristics. 
%     % \item We present a systematic study of inference heuristics by prompt-based models on different data regimes for finetuning. We study the models under two settings: (1) finetuning on varying data size from ${0,16,32,64,128,256,512}$ in which the presence of examples that support or counteract the heuristics are not controlled. \comment{0 means model is evaluated in zero-shot setting.} (2) 
% \end{itemize}

% \paragraph{Findings} Some findings that follow the hypotheses we stated above:
% \begin{itemize}
%     \item On some certain subsets of examples, zero-shot LM model does not always employ some known inference heuristics and discriminate the contrastive examples pretty well, e.g., on constituent subset of HANS and PAWS for roberta-base model. \comment{Similar behavior appear stronger in larger roberta model}.
%     \item However, once the model is exposed to more examples, the heuristics become more apparent. This indicates that the models seem to be sensitive to the few examples that support the known heuristics, i.e., few of these examples could already lead to model adapting heuristics despite good starting performance in the corresponding diagnostic datasets (see Figure \ref{fig:data_regimes}). This may well indicate how prompt-based PLM is susceptible from catastrophic forgetting \cite{McCloskey1989CatastrophicII, French1999CatastrophicFI} and to quickly specialize on the finetune dataset distribution (See illustration in Figure \ref{fig:illustration}).
%     \item Based on this observation, we propose a forgetting-aware finetuning procedure for prompt-based PLMs. Specifically, we adopt Elastic Weight Consolidation (EWC) \cite{Kirkpatrick2017OvercomingCF} to regularize the few-shot finetuning by penalizing the updates to the parameters which are crucial for the original performance \comment{which relies less on the inference heuristics}. Our results, shown in Figure \ref{fig:ewc_results1}, indicate that the diagnostic performance on HANS when PLMs fine-tuned on few-shot MNLI \cite{williams2018broad_mnli} is mantained while keeping the minimum loss on the target dataset test set. In lower data regime, e.g., 32, 64 examples, the diagnostic performance can even be improved.
%     \item Next, we highlight the importance of augmenting few counterfactual examples to the few-shot finetuning data. The results are still incomplete. However, we observe some indication that: (1) prompt-based model learn more efficiently from the smaller number of augmented examples; (2) it does well when the proportion of the examples that support and counteract the heuristics are not balanced. (3) on balanced augmentation and higher data regime, i.e., 256 training examples with 30 augmentation examples for each label; the prompt-based model demonstrate better ability to learn, as suggested by higher accuracy and more stable results on diagnostic dataset. \comment{It begs a question on whether EWC finetuning improves the learning from augmentation data even more.}
%     % show that balanced examples are needed
%     % \item Comparison with finetune across varying data regime. We show that after $n>100$, prompt-based LM learner no longer have an advantage both on the standard evaluation and heuristics diagnosis evaluation.
%     % show that finetune models could probably perform better given increasingly more frequent and balanced counterfactuals
% \end{itemize}


% \section{Discussions}
% \subsection{Impact of Counterfactuals}
% \begin{table}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|} 
% \hline
% ~~          & \multicolumn{5}{l|}{\#-support}  \\ 
% \hline
% \#-against~ & 0 & 10 & 20 & 30 & 40            \\ 
% \hline
% 10          & x & x  & x  & x  & x             \\ 
% \hline
% 20          & x & x  & x  & x  & x             \\
% \hline
% \end{tabular}
% \caption{Impact of augmenting examples that support and counteract (against) the syntactic heuristics. Each cell represent different proportion of \textit{support} and \textit{against}.}
% \end{table}
